Power-Grid Controller Anomaly Detection with Enhanced Temporal Deep Learning

Controllers of security-critical cyber-physical systems, like the power grid, are a very important class of computer systems. Attacks against the control code of a power-grid system, especially zero-day attacks, can be catastrophic. Earlier detection of the anomalies can prevent further damage. However, detecting zero-day attacks is extremely challenging because they have no known code and have unknown behavior. Furthermore, if data collected from the controller is transferred to a server through networks for analysis and detection of anomalous behavior, this creates a very large attack surface and also delays detection. In order to address this problem, we propose Reconstruction Error Distribution (RED) of Hardware Performance Counters (HPCs), and a data-driven defense system based on it. Specifically, we first train a temporal deep learning model, using only normal HPC readings from legitimate processes that run daily in these power-grid systems, to model the normal behavior of the power-grid controller. Then, we run this model using real-time data from commonly available HPCs. We use the proposed RED to enhance the temporal deep learning detection of anomalous behavior, by estimating distribution deviations from the normal behavior with an effective statistical test. Experimental results on a real power-grid controller show that we can detect anomalous behavior with high accuracy (>99.9%), nearly zero false positives and short (<360ms) latency.

==> FPGA_old.tex <==
\section{Hardware Module for Anomaly Detection}

We design a hardware module to enable the always-on anomaly detection. The module incurs minimal resource overhead by implementing only the essential computation primitives needed by LSTM inferencing and KS-test. The module is designed to be microcode-driven so that it is also programmable to support various models. We prove in the evaluation section that the module has enough performance for our detection mechanism.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{./detection_module.pdf}
    \caption{Block diagram of the hardware module}
    \label{img_blockdiagram}
\end{figure}

The architecture of our anomaly detection module is plotted in Figure~\ref{img_blockdiagram}. The processing part of the module is pipelined to have four execution stages. Look-up tables (LUTs) of non-linear functions are placed in the first execution stage. The second and third stage include multipliers (MULs) and adders (ADDs) respectively. The final execution stage is only used to latch the outputs to the external block RAM. The block RAM is a piece of addressable memory used to stored model parameters and intermediate variables during computation. The memory space of the block RAM and the address generation are managed by the microcodes of a ML/DL model. There is also a buffer to store the incoming HPC readings. The buffer is connected to the hardware module and mapped to a different region in the microcode's address space. This enables the hardware module to be programmed to fetch the input features.

The microcode is designed to instruct the datapath to perform all the necessary operation primitives. The format of a microcode is According to the introduction of LSTM model, we incorporate the following operations: 

\begin{itemize}
\item \textbf{Element-wise addition and subtraction of two vectors.} The LSTM model requires addition operation to add bias vector to a feature vector and subtraction to compute the reconstruction error. The input vectors will be forwarded to the adder stage for addition. The subtraction is computed by feeding the opposite of the second operand to the adder.

\item \textbf{Element-wise multiplication of two vectors.} Element-wise multiplication is needed by the LSTM model to combine the gates and hidden states. The input vectors will be forwarded to the multiplier stage and the product will be write back as the result.

\item \textbf{Element-wise non linear function of a vector.} Activation functions like sigmoid and tanh are used in the LSTM model. Instead of adding complicated function units to compute a fixed non-linear function, we approximate the activation functions with linear interpolation. When an input vector comes in, the slope and the intercept of a piecewise linear approximation are selected from every LUT in the first execution stage according to the input value. The slope is multiplied with the input in EXE1 stage and the intercept is added to the product in EXE2 stage.

\item \textbf{Matrix-vector multiplication.} In the LSTM model, feature vectors need to be multiplied with weight matrices. To perform this operation, the detection module first computes the element-wise products of a row in the matrix and the vector in EXE1 stage. The adders in EXE2 stage are controlled to act as an adder tree which sums up the products. As this dot product computation always takes multiple cycles to finish, the module saves repetitive read-and-refetch of partial sums by storing them in the local scratchpad. During the computation, the partial sum will be read from the local scratchpad and used as one of the inputs to the adder tree.

\end{itemize}

We also consider the operations need by the KS-test where a reference reconstruction error distribution (RED) and a test RED are compared. The reference distribution is passed to the hardware module as part of the model. The distribution parameters include a list of discrete bin boundaries and a reference cumulative histogram. We perform a KS-test for a series of computed errors by (1) adding to the a histogram defined by the discrete bin boundaries for every input error (2) computing the difference between the test histogram and the reference histogram for all the bins and (3) finding the maximum difference. To support this three-step statistical test, we need two more operation primitives which could also by computed with our hardware module:

\begin{itemize}
\item \textbf{Vector-scalar comparison.} The test error needs to be compared with every bin boundary of the reference histogram and the result will be accumulated in the test histogram. The vector scalar comparison is performed as an element-wise set-larger-than. The scalar is kept in the pipeline and the bin boundaries are streamed in for comparison. Each adder computes a difference by doing subtraction and the output is set to one if the difference is positive or zero if negative. The output could thus be understood as the histogram for one error.

\item \textbf{Find the maximum of a vector.} To find the maximum of a vector, the detection module compares the input elements in EXE2 stage by doing subtraction with the adders. A temporary maximum needs to be stored in the local scratchpad as the traversal on the vector may take multiple cycles. In each cycle, the temporary maximum is also compared with the elements being processed and gets updated until there is no other input element.

\end{itemize}

==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

\subsection{System Configuration}\label{sec:implementation:config}

We implement a prototype of our proposed detection system. Our target system is a real power-grid controller sub-system, running the real deployed power-grid controlling code. The control codes are written in Structured Text (IEC 61131-3 standard), and run on the PLC as a multi-threaded program (e.g., 23 threads as I/O, controls, etc.). The 23 threads in the Wago PLC process being monitored correspond to the main thread and 22 threads. When the PLC powers on, 7 threads are created. When an application is loaded, another 15 threads will be killed and re-spawned with a different thread ID (TID). The last thread (PLC\_Task) is the one specifically running the loaded application (utilizing the other threads to do various tasks). We list the threads and their start phase in Table \ref{tab:threads}.

%\iffalse
\begin{table}[h]
\centering
\caption{Threads running on Programmable Logic Controller}\label{tab:threads}
\scriptsize
\begin{tabular}{| C{0.2\linewidth}| C{0.7\linewidth} |}
\hline
  Start Time       & Thread(s) \\ \hline
  PLC powers on (7) & spi1, codesys3, com\_DBUS\_worker, 0ms\_Watch\_Thread, CAAEventTast, SchedExeption, Schedule \\ \hline
  Application loaded (15) & WagoAsyncRtHigh, WagoAsyncRtMed, WagoAsyncRtLow, WagoAsyncHigh, WagoAsyncMed, WagoAsyncLow, WagoAsyncBusCyc, WagoAsyncBusEvt, WagoAsyncBusEvt, WagoAsyncBusEvt, WagoAsyncBusEvt, ProcessorLoadWa, KBUS\_CYCLE\_TASK, ModbusSlaveTCP, PLC\_Task \\ \hline
  Main thread (1) & Main \\ \hline
\end{tabular}
\end{table}
%\fi

The HPCs are monitored on a real PLC with an ARM Cortex A8 processor and a custom real-time Linux distribution. Data from 4 HPCs was collected for each thread: \ding{172} the number of cycles and \ding{173} the number of instructions executed, to provide the overall running status of the thread. \ding{174} The number of L1 cache misses, to reflect the locality and temporal properties of data usage. \ding{175} The number of branch instructions, to show the changes in the control flow of the threads.

%\begin{itemize}
%\item Number of cycles executed, $N_C$
%\item Number of instructions executed, $N_I$
%\item Number of branches executed, $N_B$
%\item Number of L1 cache misses, $N_L$
%\end{itemize}


The total number of HPCs monitored is 4N if there are N threads. However, as the ARM processor has only 2 read ports, only 2 of the 4 desired HPCs are read simultaneously and then switch to read the other 2. The HPCs are sampled at 1 kHz for each of the 23 threads.

We test the system with six different real attacks in Table \ref{tab:attacks}, that are known to cause damage to the power grid. The attacks include simulating the publicly reported malicious functionalities of Stuxnet \cite{langner2011stuxnet} and BlackEnergy \cite{2015powergridattack}, i.e., halting the controller and replaying prerecorded inputs to the legitimate code. Besides, we consider other attacks against the input, output and control logic of the processor, which are the critical components of the control code. We sample 300,000 samples for each attack running.

\begin{table*}[h]
\centering
\caption{Baseline and attacks against a power-grid PLC}\label{tab:attacks}
\resizebox{\textwidth}{!}{
\begin{tabular}{| c | p{0.65\linewidth} | p{0.15\linewidth} |}
\hline
    & \textbf{Description} & \textbf{Hijack Type}\\ \hline
Baseline (Testing Normal)  & Baseline (a Proportional Integral Derivative (PID) controller) & None \\ \hline
Attack 1  & Overwrite the input (an additional line of code to overwrite the value of the input) & Input hijack \\ \hline
Attack 2  & Saturate the input (2 additional lines of code with IF condition on input value) & Control flow hijack \\ \hline
Attack 3  & Disable the PID control code (the entire PID block is commented out) & Entire Code hijack \\ \hline
Attack 4  & PID in "manual" mode (output is fixed) & Output hijack \\ \hline
Attack 5  & 2 PIDs Cascaded (input of a PID controller is sent through a second PID controller) & Control flow hijack \\ \hline
Attack 6  & Overwrite the output (an additional line of code to overwrite the value of the output) & Output hijack \\ \hline
\end{tabular}
}
\end{table*}

%\subsection{FPGA Prototype}%

%We design a minimalist yet flexible hardware module to enable the always-on anomaly detection. The module incurs minimal resource overhead by implementing only the essential computation primitives needed by LSTM inference and KS testing. The primitives of a detection model are encoded into a short program consisting of customized instructions. The short program is loaded with the model parameters into the FPGA to drive the hardware module for LSTM inference.%

%The module features a parallel architecture that does a full vector operation or matrix-vector multiply operation, over all the parallel tracks. Figure~\ref{img_blockdiagram} shows a module with four parallel tracks that loop over the matrix and vector four elements at a time. The format of a 128-bit instruction for controlling the computation is shown in Table~\ref{tbl_inst_fmt}. The~\textbf{Mode} field of an instruction defines the operation that will be performed by the datapath pipeline. A single instruction invokes a multi-cycle execution in this mode for the entire length of the vector or size of the matrix depending on the ~\textbf{Length} and ~\textbf{Width} fields.%

%%The module is driven by this program so that it is also programmable to support various models.%

%\iffalse
%\begin{table}[ht!]
%\centering
%\caption{Format of instructions read by the hardware module}
%\label{tbl_inst_fmt}
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%\textbf{Inst} & \textbf{{[}127:124{]}} & \textbf{{[}123:110{]}} & \textbf{{[}109:96{]}} & \textbf{{[}95:64{]}} & \textbf{{[}63:32{]}} & \textbf{{[}31:0{]}} \\ \hline
%\textbf{Field} & \textbf{Mode}              & \textbf{Length}            & \textbf{Width}            & \textbf{Addr\_X}         & \textbf{Addr\_Y}         & \textbf{Addr\_Z}        \\ \hline
%\end{tabular}
%\end{table}
%\fi%

%\begin{table}[ht!]
%\centering
%\caption{Format of instructions read by the hardware module}\label{tbl_inst_fmt}
%\resizebox{0.5\textwidth}{!}{
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%\textbf{Inst{[}127:124{]}} & \textbf{Inst{[}123:110{]}} & \textbf{Inst{[}109:96{]}} & \textbf{Inst{[}95:64{]}} & \textbf{Inst{[}63:32{]}} & \textbf{Inst{[}31:0{]}} \\ \hline
%\textbf{Mode}              & \textbf{Length}            & \textbf{Width}            & \textbf{Addr\_X}         & \textbf{Addr\_Y}         & \textbf{Addr\_Z}        \\ \hline
%\end{tabular}
%}
%\end{table}%

%%Table~\ref{tbl_inst_fmt} shows the 128-bit instruction format. The~\textbf{Mode} field defines the memory-to-memory operation that will be performed by the detection module. The~\textbf{Length} and~\textbf{Width} fields control the number of times for which the operation will be repeated. For a element-wise vector operation, the \textbf{length} field is set to be the length of input vector(s). In a matrix-vector operation,~\textbf{Length} and~\textbf{Width} represent the matrix size. An instruction taking multiple cycles to finish will stay in the pipeline until the counter of executed loops in the~\textbf{Decode} stage reaches the number specified by the~\textbf{Length} and~\textbf{Width} fields. Moreover, the module memory-to-memory operation%

%\begin{figure}
%    \centering
%    \includegraphics[width=0.9\linewidth]{./figures/detection_module.pdf}
%    \caption{Block diagram of the anomaly detection module}
%    \label{img_blockdiagram}
%\end{figure}%

%%The architecture of our anomaly detection module is plotted in Figure~\ref{img_blockdiagram}. The processing part of the module is pipelined with four execution stages. Look-up tables (LUTs) of non-linear functions are placed in the first execution stage. The second and third stages include multipliers (MULs) and adders (ADDs) respectively. The final execution stage is only used to latch the outputs to the external block RAM. Our design supports parallel processing and a current prototype has 4 parallel computing tracks, each having one LUT, one multiplier and one adder. %

%Unlike other vector units, we use a memory-to-memory architecture rather than vector registers. We believe this gives a more flexible and simpler architecture. We use a software-managed memory, where we can lay out the memory contents based on matrix and vector sizes. We refer to operands by their addresses in this memory in the instruction.  In our FPGA implementation, the BRAM (block RAM) is used as the software-managed memory with 32 bits of address space.
%%The architecture also performs vector operations in a memory-to-memory manner where we use a software-managed memory instead of vector registers. The operands are specified by their addresses in the instructions, which gives a more flexible architecture for efficiently implementing different algorithms without the complexity to manage the register. In our FPGA prototype implementation, the block RAM is used to store model parameters and intermediate variables during computation.
%%The memory space of the block RAM and the address generation are managed by the instructions of an ML/DL model for anomaly detection.
%There is also a buffer to store the HPC readings. The buffer can be accessed by the hardware module to load the incoming reading for anomaly detection.%

%%the software-defined memory stores the matrices, vectors and other parameters of the LSTM model, and is implemented in the FPGA’s local BRAM memory.  A chunk of this local memory is also reserved for double buffering of the inputs (in this case the HPC values for a window for prediction), so that one buffer is being used for the LSTM inferencing and KS testing while the other buffer is being filled from the new HPC values.%

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=\linewidth]{./figures/lstm_combined.pdf}
%    \caption{An LSTM cell (top) and mapping LSTM inference to our FPGA instructions (bottom). %For $*=f, i, o, n$, the weight matrices, $W_*$ and $U_*$, and the biases, $b_*$, %used to compute $PreAct_* (*=f, i, o, n)$ are concatenated as
%    }
%    \label{img_lstm_eq_fig}
%\end{figure}%

%\subsubsection{Support for LSTM Inference} ~\\
%Figure~\ref{img_lstm_eq_fig} shows an LSTM cell (top), and the operations used in LSTM inference. Model weights denoted by $W_* (* = f,i,o,n,p)$ and $U_* (* = f,i,o,n)$ are matrices and the biases denoted by $b_* (* = f,i,o,n,p)$ are vectors. Their sizes are hyper-parameters of the DL model. %Although an LSTM cell needs 8 matrix-vector multiplications and 8 vector-vector additions to
%When computing $PreAct_* (* = f,i,o,n)$ in an LSTM cell, we optimize by concatenating the weight matrices, $W_*$ and $U_*$, and biases, $b_*$, into one large matrix to multiply with the concatenation of $x_t$, $h_{t-1}$ and $1$. This combination reduces the number of instructions from 8 matrix-vector multiplications and 8 vector additions to 1 matrix-vector multiplication. There are also vector additions, multiplications and 5 non-linear activation functions. % to compute a prediction, $P_{t+1}$, as the output at time t.
%These operations are common to other deep learning and machine learning algorithms. Hence we implement the following operation modes in the execution stages of the parallel datapath.%

%\bheading{Vector-vector operations.} The module can perform element-wise vector-vector operations like vector multiplication (\textbf{Vmul}) in EXE1 stage, or vector addition (\textbf{Vadd}) or subtraction (\textbf{Vsub}) in EXE2 stage.%

%%input vectors will be forwarded to the EXE2 stage for addition (\textbf{Vadd}). Subtraction (\textbf{Vsub}) is computed by feeding the negative of the second operand to the adder.%

%%\bheading{Element-wise multiplication of two vectors.} In vector multiplication mode (\textbf{Vmul}), the input vectors will be forwarded to the multiplier stage EXE1.%

%\bheading{Non-linear activation functions of a vector.} The LSTM model needs a vector activation mode (\textbf{Vact}) to compute non-linear functions, e.g. sigmoid and tanh. Rather than adding complicated functional units, we use linear interpolation to approximate the activation functions. When an input vector comes in, the slope, slp[i], and the intercept, b[i], of a piecewise linear approximation are read from a selected entry in a look-up table (LUT) in EXE0 stage according to the input value, X[i]. The result, Z[i], is computed in the following two stages (EXE1 and EXE2) as $Z[i] = slp[i] \times X[i] + b[i]$. %Different from \cite{Chen:2014:DSH:2541940.2541967} where the non-linear units are placed in the last stage, requiring extra multipliers and adders, our design reduces the function units by placing the LUTs in an earlier stage so that existing multipliers and adders in later stages are reused.%

%\bheading{Matrix-vector multiplication.} %In the LSTM model shown in Figure~\ref{img_lstm_eq_fig}, the~\textbf{MVmul} mode is needed to multiply feature vectors, e.g. $x_t$ and $h_t$, with weight matrices, e.g. $W_f$ and $U_f$.
%The datapath computes the multiply-accumulate operation with the multipliers and adders in EXE1 and EXE2 stages. We adopt loop tiling for matrix-vector multiplication \cite{Chen:2014:DSH:2541940.2541967} \cite{song2018situ} to reduce memory traffic by unrolling a loop and increasing data reuse. We optimize by adding a local scratchpad memory in EXE2 stage to save repetitive store-and-reload of partial sums in the multiplication from block RAM and reduce the read latency by temporarily storing the partial sums in the local scratchpad memory. We also optimize by making the adders in EXE2 stage controllable to act as an adder tree so that no extra adders are needed. During the computation, the partial sum is read from the local scratchpad and used as one of the inputs to the adder tree.%

%%\textbf{\ding{172} Adder reuse.} Without adding more adders to sum up the products, we make the adders in EXE2 stage controllable to act as an adder tree which takes the products and the previous partial sum as its input.%

%\iffalse
%\begin{figure}[h]
%\begin{lstlisting}[language=C, frame=single, xleftmargin=.5em, framexleftmargin=.5em, caption={Tiling for Matrix-vector Multiplication}, label={alg_tiling}]
%  // N_local: size of local scratchpad
%  // N_track: number of parallel computing tracks
%  for (i = 0; i < L; i+= N_local)
%    for (j = 0; j < W; j += N_track)
%      for (ii = 0; ii < N_local; ii ++)
%        // Computed every cycle
%        for (jj = 0; jj < N_track; jj++)
%          O[i*N_local+ii] += W[i*N_local+ii][j*N_track+jj] * I[j*N_track+jj]
%\end{lstlisting}
%\end{figure}
%\fi%

%\iffalse
%\begin{figure}[h]
%\begin{lstlisting}[language=C, frame=single, xleftmargin=.5em, framexleftmargin=.5em, caption={KS-test Implementation}, label={alg_kstest}]
%  // Step 1: Get testing cumulative histogram
%  for (i = 0; i < L_test; i++)
%    for (j = 0; j < L_ref; j ++)
%      // Need vector-scalar comparison
%      if test_err[i] < ref_bin[j]
%        test_hist[j]++
%
%  // Step 2: Compare with reference histogram
%  for (i = 0; i < L_ref; i++)
%    diff_hist[i] = ref_hist[i] - test_hist[i]
%
%  // Step 3: Find maximum difference
%  // Need to find the maximum in a vector
%  diff_max = max(diff_hist)
%
%  // Step 4: Report result
%  if (diff_max > diff_th)
%    report_anomaly(diff_max)
%  else
%    report_normal(diff_max)
%\end{lstlisting}
%\end{figure}
%\fi%

%\subsubsection{Support for Statistic Test} ~\\
%KS test determines whether the reference RED and the observed RED are the same distribution. The reference RED is collected in the training phase and represented by reference bin boundaries and a reference cumulative histogram. The observed RED is collected online and represented by a series of observed errors. %

%We implement a five-step KS test module on FPGA and show an example of the workflow in Figure \ref{fig:ks_test}. The grey dotted boxes represent inputs and output. Step \ding{172}: compare an observed error with bin boundaries. The output of this step is a vector of ``0''s and ``1''s. ``1'' represents that the observed error is less than the corresponding bin boundary, and ``0'' otherwise. This step requires a new operation for vector-scalar comparison (\textbf{VSslt}). Step \ding{173}: accumulate all binary vectors from \ding{172}. The accumulated vector, namely ``observed histogram'', conceptually represents the cumulative histogram of the observed errors using the reference bins. Step \ding{174} and step \ding{175}: find the largest difference in the reference and observed histograms, i.e. KS statistics $D_{n,m}$ in Eq (\ref{equ:KSstatistic}). Step \ding{174} is a vector subtraction and step \ding{175} is a new operation, \textbf{Vmaxabs}, to find the maximum absolute value in a vector. Step \ding{176}: compare $D_{n,m}$ with a threshold, i.e. RHS of Eq (\ref{equ:KStestinequ}), to determine normality. A \textbf{VSslt} instruction with a vector size of 1 is used for the scalar-scalar comparison in step \ding{176}. Hence, we introduce two new operation modes, \textbf{VSslt} and \textbf{Vmaxabs}, to support KS testing:%

%%we perform a KS test for a series of computed errors by~\circled{1} getting the cumulative histogram of the current test error, ~\circled{2} adding the histogram of every input error to the test histogram,~\circled{3} computing the difference between the testing and the reference histograms,~\circled{4} finding the maximum absolute difference and~\circled{5} comparing it with a predefined threshold. To support this five-step statistical test, we add two more operation primitives,~\textbf{VSslt} and~\textbf{Vmaxabs}, which are mentioned in Figure~\ref{img_ks_test}:%

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=0.9\linewidth]{./figures/ks_test.pdf}
%    \caption{An example of five-step KS test. Two new operation primitives, \textbf{VSslt} and \textbf{Vmaxabs}, are implemented in step \ding{173} and \ding{175} to support KS test, respectively.}
%    \label{fig:ks_test}
%\end{figure}%

%%circled{2}: needs~\textbf{Vadd} to accumulate the histogram of current error in the test histogram and it is already implemented for LSTM. The comparison with reference histogram in~\circled{3} requires~\textbf{Vsub} which has also been supported.~\circled{4} uses~\textbf{Vmaxabs} mode to find the maximum of absolute histogram difference, namely the $D_{n,m}$ in Eq~(\ref{equ:KSstatistic}).~\circled{5} computes Eq~(\ref{equ:KStestinequ}) with another~\textbf{VSslt} instruction with a length of one to compare $D_{n,m}$ with the threshold.}%

%\bheading{Vector-scalar comparison.} The vector-scalar comparison mode,~\textbf{VSslt}, sets an output element to one if the scalar is less than the corresponding element in the input vector. During execution, the scalar is kept in the pipeline, and the bin boundaries are streamed in for comparison. Each adder does subtraction, and the output is decided by the sign of the difference.
%%This operation mode can also be used for the scalar-scalar comparison with threshold in Step 3.
%%The output could thus be treated as the histogram for one error. %

%\bheading{Find the maximum absolute value in a vector.} In~\textbf{Vmaxabs} mode, the datapath compares the absolute values of input elements in EXE2 stage by doing subtraction with the adders. A temporary maximum is stored in the local scratchpad as the loop on the vector can take multiple cycles to finish. Every cycle the temporary maximum is compared with the maximum of absolute values and gets updated.


==> intro_backup.tex <==
\section{Introduction}\label{sec:intro}

The power-grid is a critical infrastructure, and attacks on it can cripple society, affecting national security, economic competitiveness and societal interactions. In 2015, Ukraine experienced cyber attacks against its power-grid system \cite{2015powergridattack}. During this attack, 30 substations were switched off and 230 thousand people were left without electricity. The U.S. Government Accountability Office (GAO) questioned the current adequacy of defenses against power-grid attacks, and the North American Electric Reliability Corporation (NERC) has recognized these concerns \cite{sridhar2012cyber}. With power-grid substations controllable through cyberspace transactions, the concern about cyber attacks on the physical power-grid systems is a real and serious threat, which is the focus of our paper. Although these attacks can have disastrous impact, they are still an unsolved problem.

There have been detection approaches proposed to protect the power-grid system by examining the physical sensors. Manandhar \cite{manandhar2014detection} used Kalman filters to model the voltage sensors and $\chi^2$ test to detect physical anomalies in the power-grid system. Valenzuela \cite{valenzuela2013real} used Principle Component Analysis (PCA) and irregular-space analysis to detect anomalies in the power-grid. Cardenas \cite{cardenas2011attacks} suggested using linear models and threshold random walk (TRW) to deal with the unseen attacks. Zhao \cite{zhao2014real} proposed an expert system with Hidden Semi-Markov model. However, they may have oversimplified system behavior in their model, meanwhile only focused on the algorithms but neglected the system design. Previous work on the cyber-security of power-grid systems focus on protecting the networks and data transmission \cite{wang2011security, sikdar2011defending, zhang2011distributed}. Each of these solved a specific loophole of secure communication in the power-grid system, but can hardly guarantee the detection of new attacks.

%proposed a secure wireless communication architecture in the power-grid stations. Fouda \cite{fouda2011lightweight, zhang2011distributed}. proposed an authentication scheme for communications in the context of a power-grid system. Sikdar \cite{sikdar2011defending} protected the anonymity of data to defend against the power-grid traffic analysis attacks. Zhang \cite{zhang2011distributed} used SVM at different levels of the power-grid system to detect network anomalies. Each of these solved a specific loophole of secure communication in the power-grid system, but can hardly guarantee the detection of new attacks.

%There have been other detection approaches proposed to protect the power-grid system by examining the physical sensors. Manandhar \cite{manandhar2014detection} used Kalman filters to model the voltage sensors and $\chi^2$ test to detect physical anomalies in the power-grid system. However, their model assumed simple sine wave inputs which cannot be extended to a broader scope of sensor readings. In addition, the electrical sensor readings could be spoofed by the adversary \cite{kune2013ghost}. Valenzuela \cite{valenzuela2013real} used Principle Component Analysis (PCA) and irregular-space analysis to detect anomalies in the power-grid. However, they may have oversimplified the problem by assuming the anomalies lie in a subspace of the input data space. Cardenas \cite{cardenas2011attacks} suggested using linear models and threshold random walk (TRW) to deal with the unseen attacks. However, their proposed linear models are too simple to reflect the real complex physical processes. Zhao \cite{zhao2014real} proposed an expert system with Hidden Semi-Markov model. Their system requires the interaction between experts, thus it could be biased by the human experience of the known attacks.

Besides the sensors and network, protecting the control code running on the industrial programmable logic controllers (PLCs) is an essential and fundamental task in protecting the power-grid systems. No matter how the adversary spreads the malware or bad programs through system vulnerabilities, his ultimate goal is taking control of the power-grid infrastructures, destroying them or turning them off, and thus inducing huge physical impact. This attack strategy has been shown in the Stuxnet \cite{langner2011stuxnet} and BlackEnergy \cite{2015powergridattack} attacks. Therefore, rather than physical attacks on the physical power-grid system, we consider cyber attacks that hijack the controller code that controls the actuators of the physical system.

However, the protection of controllers in the power-grid system against zero-day attacks has not had much attention in the computer architecture community so far. It is challenging because \ding{172} there is no prior-knowledge about the attacks, especially in the realistic "zero-day" attack settings. \ding{173} Various controllers, e.g. ABB, Siemens and Wago, and OS, e.g. Windows, Unix and proprietary OS (SIMATIC WinCC), are widely used in modern power-grid systems, exposing a large attack surface. \ding{174} The power-grid systems usually implement weak anti-virus and integrity checking mechanisms on both executed code and transferred data, due to the computation capacity and hard-realtime constraints \cite{humayed2017cyber}. \ding{175} Many concurrent threads are running on the controller simultaneously. Stealthy attack programs that have infected the controller can hide within these threads. \ding{176} Previous anomaly detection approaches transfer the data to a central server through network, introducing a large attack surface and long latency.

%However, the protection of controllers in the power-grid system against zero-day attacks has not had much attention in the computer architecture community so far. It is challenging because \ding{172} there is no prior-knowledge about the attacks, especially in the realistic "zero-day" attack settings. Labeled attack data are highly sensitive and not available for training. \ding{173} Various controllers, e.g. ABB, Mitsubishi, Siemens and Wago, and OS, e.g. Windows, Unix and proprietary OS (SIMATIC WinCC), are widely used in modern power-grid systems, exposing a large attack surface. \ding{174} The power-grid systems usually implement weak anti-virus and integrity checking mechanisms on both executed code and transferred data, due to the computation capacity and hard-realtime constraints \cite{humayed2017cyber}. For example, runtime code integrity checking \cite{seshadri2005pioneer, seshadri2007secvisor} cannot be directly applied to power-grid systems, because of the high overhead in a real-time system. \ding{175} Many concurrent threads are running on the power-grid controller simultaneously. Stealthy attack programs that have infected the controller can hide within these threads. Dolgikh \cite{dolgikh2012using} proposed customized normalcy profiles for programs in the power-grid systems, but they assumed that there are only limited applications running in the system.

%However, they proposed no specific defense techniques against the attacks.

%The hijacking of controllers in power-grid systems, could become the next security nightmare. We summarize the characteristics making power-grid systems vulnerable to the controller hijacking attacks. First, \red{Second, different Operating Systems (OS), including general-purpose OS (Windows and Unix) and proprietary OS (SIMATIC WinCC), running on the power-grid systems, amplifies these threats.} Third, power-grid system itself usually implements weak anti-virus and integrity checking mechanisms on both executed code and transferred data, due to the power and spatial constraints \cite{humayed2017cyber}. Fourth, attacks on the controllers of these power-grid systems could cause devastating physical damage.}

%Cyber-physical systems are deployed in many areas, including the sensing and control of energy, health-care, civil infrastructure, transportation and entertainment systems. Representative examples of cyber-physical systems are the smart power grid \cite{fang2012smart}, water treatment systems \cite{lin2009towards}, Carbon Dioxide monitoring system to support green transportation \cite{froehlich2009ubigreen}, heart disease monitoring system \cite{leijdekkers2006personal}, autonomous driving system \cite{berger2014autonomous} and a distributed autonomous gardening system \cite{correll2009building}.

%Unfortunately, the attacks against CPS, including power-grid systems, not just stay in the lab, but have already been realistic and caused massive losses. They can result in large-scale physical damage. For example, Stuxnet hijacked centrifuges controllers \cite{langner2011stuxnet}. The hijacking of medical devices results in loss of patients' privacy \cite{MedicalDeviceHijack1} \cite{MedicalDeviceHijack2}. Recently autonomous cars \cite{hackjeep} and drones \cite{son2015rocking} have also been hijacked and controlled remotely.

%On the other side, luckily, the designs of CPS under resource constraints provide us with a chance to investigate specific defenses otherwise not applicable to general-purpose systems. Our key observation is, the controller behaviors in CPS are more deterministic and \textbf{predictable} than general-purpose systems. We investigate through a large-scale experiment on the controllers in a real power grid system to justify our findings. With this insight, we propose a novel and universal data-driven approach to address the problem of attacks, including \textbf{zero-day} attacks in the cyber-physical systems. Our proposed defense does not require any information about the attacker.

%Our approach is specifically designed for cyber-physical systems. First, an OS is not compulsory in our defense, in contrast to complicated general-purpose defense with full OS support \cite{shacham2004effectiveness} \cite{pappas2012kbouncer} \cite{cowan1998stackguard}. Second,

In this paper, we propose a new data-driven architecture to detect zero-day controller hijacking attacks on power-grid systems. Our proposed defense provides comprehensive and reliable protection against unknown attacks. It does not look for specific attacks or triggers, but rather a holistic view of controller operation. Specifically, our proposed approach first automatically learns the normal behavior of the controller using temporal deep learning, and generates a corresponding behavioral model of the controller. Then we use the generated model, enhanced by an effective statistical test to detect the deviation from processor normal behavior through \textit{reconstruction error distribution (RED)}. We design a minimalist yet flexible FPGA implementation that can be added in the controller and show that this can implement the deep learning and statistical inferencing required, resulting in a more secure and faster anomaly detection system.

Our main contributions in this paper are:

%Earlier detection of the anomalous controller behavior can help quick mitigation and recovery from the attack, for example, switching to a safe but not up-to-date version of the control code.

%We propose a data-driven architecture that first trains a temporal deep learning model, using only normal data from legitimate processes that run daily in these power-grid systems, to model the normal behavior of the power-grid controller. Then, we run this model in the power plant using real-time data collected from commonly available hardware performance counters. We propose a new way to quickly detect if malicious code is running on the processor, by estimating deviations from the normal behavior with an effective statistical test. We design a minimalist yet flexible FPGA implementation that can be added in the controller and show that this can implement the deep learning and statistical inferencing required. This results in both a more secure and faster anomaly and attack detection system. Experimental results on a real power-grid controller show that we can detect anomalous behavior in real-time with high accuracy and nearly zero false positives.


\begin{itemize}
%\item We observe that the controller behavior in the power-grid systems are predictable to some degree, because the hard-realtime control events come up in a periodic way.

\item We propose a new data-driven, learning-based, statistically-enhanced architecture for detecting anomalies in the power-grid controllers. Intuitively, this defense predicts the future behavior of the controller through a well-trained deep temporal model and low-cost hardware performance counter features, and investigates the reconstruction error distribution (RED). No prior-knowledge of attacks is needed in either the training or inference, thus it can be used to detect zero-day attacks.

\item We implement an FPGA prototype of our defense system. It reduces the network transaction overhead and attack surface of transferring data to a central server for processing.

\item We evaluate our proposed defense on real power-grid controllers in multiple dimensions, by simulating the publicly reported attack functionalities \cite{langner2011stuxnet, case2016analysis}, to show the superiority of our proposed solution.
%Experiment show that we achieve high accuracy with short latency.
%We achieve low latency, high accuracy with nearly zero false positives.
%We also compare it with conventional anomaly detection approaches.
\end{itemize}

In Section \ref{sec:background}, we provide background on the power-grid system, Program Logic Controllers (PLCs), hardware performance counters features and statistical test we use in our defense. In Section \ref{sec:SecurityConsiderations}, we articulate our threat model. In Section \ref{sec:solution}, we present our architecture in detail. In Section \ref{sec:implementation}, we show our implementation. In Section \ref{sec:PerformanceEva} and \ref{sec:AccuracyEva}, we present the performance and accuracy evaluation, respectively. We discuss related work in Section \ref{sec:relatedwork} and conclude in Section \ref{sec:conclusion}.


==> performance.tex <==
\section{Performance and Storage Evaluation}\label{sec:PerformanceEva}
\subsection{Performance Evaluation}

Figure \ref{fig:timing} details the time taken by our LSTM+KS architecture to detect an anomaly.

\bheading{\ding{172} LSTM Prediction Time $t_{predict}$.} This is the inference time for the LSTM model to predict the controller behavior, in terms of the HPC values for one reading.

\bheading{\ding{173} Sampling Interval $t_{sample}$.} This is the interval between two HPC readings.
%The accumulated number of corresponding hardware events are stored in the HPCs during the interval.

\bheading{\ding{174} Error Accumulation (EA) Time $t_{EA}$.} This is the time to gather one point of the reconstruction error. Note that in Eq (\ref{equ:reconstructionerror}), one point of the reconstruction error is accumulated among $L$ time frames. Therefore, $t_{EA}=max\{t_{predict}, t_{sample}\}\times L$.

\bheading{\ding{175} RED Collection Time $t_{RED}$.} This is the time to collect the testing reconstruction error distribution. This distribution is represented by $N_{EA}$ independent reconstruction errors in \ding{174}.

\bheading{\ding{176} KS-Test Time $t_{KS}$.} This is the time to compute the KS statistic and determine if an anomaly has occurred.

\begin{figure}[h]
 \centering
  \includegraphics[width=\linewidth]{figures/timing.pdf}
  \caption{Latency evaluation for our proposed architecture.}
  \label{fig:timing}
\end{figure}

%Furthermore, updating the model is faster than training from scratch. Therefore, we evaluate the time for training the model from scratch, and the latency for online detection.

%In each inference time period, we can infer multiple PLC sequences in parallel. 

%We can parallelize 256 PLC sequences, the degree of parallelization depends on the GPU we are running on. For each time frame, we need to predict 2000 time stamps in the future and subsample it, to ensure the independence required by KS test samples. Thus, the time taken to detect an attack is 2 seconds (2000 / 1 kHz), i.e. if an attack happens at $t$ seconds, it can be discovered at $t+2$ seconds as anomalous PLC behavior. In a real implementation, a trusted deep learning accelerator can be used (Figure \ref{fig:system}), which will give faster execution time and greater security through hardware isolation.

The detection latency $t_{detection}$, i.e. the time interval between the occurrence of the attack and the detection of the anomaly, is determined by $L, N_{EA}$ in the algorithm, and $t_{predict}$, $t_{sample}$ and $t_{KS}$ in the real implementation. Specifically,
\vspace{-0.1cm}
{\small
\begin{align}
t_{detection}&= t_{RED}+t_{KS} \label{eq:tRED} \\ 
&= max\{t_{predict}, t_{sample}\}\times L\times N_{EA} + t_{KS}
\end{align}
}%
\vspace{-0.5cm}

We observe that $t_{RED}$, proportional to $L \times N_{EA}$, dominates $t_{KS}$ in Eq (\ref{eq:tRED}). Thus we look for the minimal $L \times N_{EA}$ that maintains false positives rate (FPR) $<10^{-4}$. We start with L = 50 and $N_{EA}$ = 40 to give a detection time of about 2 seconds. Then, through trial-and-error, we reduce L or $N_{EA}$, while holding FPR $<10^{-4}$. We observe a significant FPR increase ($\sim$10.4\%) after $L \times N_{EA}$ = 250. Hence, we choose $L=10$ and $N_{EA}=25$ in our implementation.

%\begin{figure}[h]
% \centering
%  \includegraphics[width=0.8\linewidth]{figures/NL.pdf}
%  \caption{The highest accuracy for each $N_{EA}*L$. We observe a significant drop when $N_{EA}*L<200$. At this point, $L=25$ and $N_{EA}=10$}
%  \label{fig:NL}
%\end{figure}

The FPGA prototype is running at 125MHz and it has enough performance for our detection mechanism. Other implementations can increase the number of parallel tracks according to the target workload. We show our FPGA time measurements in Table \ref{tab:performance} row 1. We also implement the anomaly detection with data transferred to an application server (Figure \ref{fig:SCADA}) with a GPU, for comparison with our in-situ FPGA implementation, in row 2 of Table \ref{tab:performance}. For this, we implement the LSTM model on an Nvidia 1080Ti GPU. The server is equipped with 2 Intel Xeon E5-2667 2.90GHz CPUs, each with 6 cores, running on Ubuntu 14.04.5 LTS. The level 1 instruction and data caches are 32 KB, the level 2 cache is 256 KB and the level 3 cache is 16MB. 

We observe that $t_{predict} < t_{sample}$ using both the FPGA and GPU implementation, i.e. the bottleneck is the HPC sampling. However, note that using the server GPU introduces extra network transaction time $t_{network}$=100 ms round-trip. Training is typically done off-line only once on the application server, and needs to be updated only if the functionality of the control code is modified, while only inferencing is needed in real-time.

\vspace{-0.5cm}
\begin{table}[h]
\centering
\caption{Execution time for model training and inferencing, and KS testing, for detecting controller anomalous behavior. In both implementation, $L=25$ and $N_{EA}=10$.}\label{tab:performance}
\resizebox{\linewidth}{!}{
\begin{tabular}{| c | c | c | c | c | c | c | c | c |} 
\hline
     & \textbf{Training}  & $t_{network}$ & $t_{sample}$ & $t_{predict}$ & $t_{EA}$     & $t_{RED}$ & $t_{KS}$         & \textbf{Detection} \\ \hline
\textbf{FPGA} & --   & --         & 1 ms         & 0.17 ms       & 25 ms        & 250 ms    &   10$\mu s$      & \textbf{250 ms}          \\ \hline
\textbf{GPU}  & \textbf{21.1 min}   & 100 ms   & 1 ms         & 0.53 ms       & 25 ms        & 250 ms    &   8.6 ms ${}^\star$ & \textbf{358.6 ms}        \\ \hline
\end{tabular}
}
\begin{tablenotes}
    \scriptsize
    \item ${}^{\star}$ KS test is implemented on the server CPU.
\end{tablenotes}
\end{table}
\vspace{-0.5cm}

\subsection{Storage and FPGA requirements}
The trained deep learning model and the reference RED need to be stored. In our FPGA implementation, the deep learning model is an LSTM with 128 hidden nodes, 325.1KB in size. The reference RED is less than 1KB in size. In total, we need $<$ 326 KB storage, which fits in our FPGA BRAM memory. Our implemented detection module, equipped with four computing tracks, uses 6.5k FPGA LUTs, 4.2k FPGA flip-flops, 16 DSPs and 281 block RAM units. Compared to other published FPGA designs for LSTM computation \cite{gao2018deltarnn}, our LSTM detection module uses much fewer FPGA resources, while still providing enough performance for anomaly detection in power-grid systems.

%performance-oriented designs for LSTM computation \cite{gao2018deltarnn}, the detection module provides enough performance for anomaly detection in power-grid systems, but uses 40.2X, 28.4X, 48X and 1.63X fewer corresponding resources. 

%It shows a trade-off of hardware support for DL applications when the performance is not the only dominating factor to consider.

%Our implemented detection module, equipped with four computing tracks, uses 6.5k FPGA LUTs, 4.2k FPGA flip-flops, 16 DSPs and 281 block RAM modules, i.e. 40.2X, 28.4X, 48X and 1.63X fewer than performance oriented design for LSTM computation \cite{gao2018deltarnn}. It demonstrates a trade-off of hardware support for DL applications when the performance is not the only dominating factor to consider.

%\begin{table}[h]
%\centering
%\caption{Execution time for model training and inferencing, and KS testing, for detecting the controller hijacking attacks.}\label{tab:performance}
%\resizebox{0.6\linewidth}{!}{
%\begin{tabular}{| c | c | c | c |} 
%\hline
%       & Training & Inference & KS Test \\ \hline
%LSTM & 21.1 min & 39.8 ms & 8.63 ms \\ \hline
%CRBM & 3.5 min & 265 ms & 8.63 ms \\ \hline
%\end{tabular}
%}
%\end{table}


==> prediction.tex <==
\section{Predictability of Controller Behavior in CPS}\label{sec:observation}

\subsection{Our Insights}

In order to address the first challenge, we decide to use hardware performance counters as our behavior indicator. Though modern OS supports high-level APIs for reading the HPC values, we can also read them from bare-metal CPS. HPCs record the performance of the program running on the controller, thus they also provide valuable information about the behavior of the controller. Another advantage is that HPCs as hardware registers are hard to tamper with.

The second challenge is addressed by our observation that the controller behavior are highly predictable. Therefore, we can train a deep learning model to learn the normal behavior distribution of the controller. A deviation from the learned distribution indicates the controller code is likely to be hijacked.

In order to decrease the false positives due to the third challenge, we are inspired by the fact that different distributions can be distinguished by statistical tests, such as the t-test and the Kolmogorov-Smirnov (KS) test. We use deep temporal model in combination of the KS test to improve the accuracy. If the processor behaves normally, the behaviors are highly predictable by a trained deep temporal model. The model predictions and real observations are supposed to be close (small differences). On the other hand, if the controller code is hijacked, there would be large differences between the normal predictions and hijacked real observations. Thus, determining whether the differences are from the same distribution by using statistical testing is equivalent to controller code hijacking detection.

%\begin{enumerate}
%\item Normal programs and processor behavior are predictable by using history behaviors. There are strong relations between previous and future program instructions executed, although the relations are implicit and need to be explored.
%\item A sequence predictor, trained on baseline (normal) behaviors, will have different prediction error distributions when comparing HPC measurements of abnormal sequences with predicted normal sequences. In general, the errors are larger for abnormal sequences.
%\end{enumerate}

\subsection{Large-scale Experiment Verification}

To verify the correctness of our observation that controller behavior are predictable, we collect 300,000 samples from 4 HPCs readings of 23 threads on a real daily-run power grid system. We find 40 HPCs values for specific threads are always zeros, and we exclude these HPC values and train an LSTM to predict its controller behavior in terms of HPCs.

We use Signal-to-Noise ratio (SNR) as our measurement of the quality of our prediction. Without complicated feature selection and preprocessing, on this large dataset we are able to achieve \textbf{average SNR = 12.68 dB}. Note that random guesses result in SRN very close to $-\infty$, thus this SNR indicates that the controller behavior are highly predictable in terms of HPCs in CPS.

